Active Learning for Control-Oriented Identification of Nonlinear Systems

Model-based reinforcement learning is an effective approach for controlling an unknown system. It is based on a longstanding pipeline familiar to the control community in which one performs experiments on the environment to collect a dataset, uses the resulting dataset to identify a model of the system, and finally performs control synthesis using the identified model. As interacting with the system may be costly and time consuming, targeted exploration is crucial for developing an effective control-oriented model with minimal experimentation. Motivated by this challenge, recent work has begun to study finite sample data requirements and sample efficient algorithms for the problem of optimal exploration in model-based reinforcement learning. However, existing theory and algorithms are limited to model classes which are linear in the parameters. Our work instead focuses on models with nonlinear parameter dependencies, and presents the first finite sample analysis of an active learning algorithm suitable for a general class of nonlinear dynamics. In certain settings, the excess control cost of our algorithm achieves the optimal rate, up to logarithmic factors. We validate our approach in simulation, showcasing the advantage of active, control-oriented exploration for controlling nonlinear systems.

==> tex/problem_formulation_copy.tex <==
\section{Problem Formulation}
\label{s: problem formulation}


We consider a nonlinear dynamical system evolving according to 
\begin{align}
    \label{eq: dyn}
    X_{t+1} = f(X_t, U_t; \phi^\star) + W_t, \quad t=1,\dots T,
\end{align}
with state $X_t$ assuming values in $\R^{\dx}$,  input $U_t$ assuming values in $\R^{\du}$, and $\dx$-dimensional noise $W_t \overset{\iid}{\sim} \calN(0, \sigma_w^2 I)$. For simplicity, we assume $X_1 = 0$. Here, $f$ is the dynamics function, which depends on an unknown parameter $\phi^\star \in \R^{d_{\phi}}$. We assume that there exists some positive $B$ such that 
$\norm{f(\cdot, \cdot, \phi)}_\infty \leq B$ for all $\phi \in \R^{d_{\phi}}$ . 

We study a learner whose objective is to determine a policy $\pi = \curly{\pi_t}_{t=1}^T$ from a policy class $\Pi^\star$ to minimize the cost $\calJ(\pi, \phi^\star)$, where
\begin{align}
    \label{eq: objective}
    \calJ(\pi, \phi) = \E_{\pi}^{\phi} \brac{\sum_{t=1}^T c_t(X_t, U_t) + c_{T+1}(X_{T+1})}.
\end{align}
The superscript on the expectation denotes that the dynamics \eqref{eq: dyn} are rolled out under parameter $\phi$, while the subscript denotes that the system is played in closed-loop under the feedback control policy $U_t = \pi_t(X_1, U_1, \dots, X_{t-1}, U_{t-1}, X_t)$ for $t=1,\dots,T$. The learner follows a two step interaction protocol with an exploration phase, and an evaluation phase. In the exploration phase, the learner interacts with the system for a total of $N$ episodes, each consisting of $T$ timesteps, by playing exploration policies $\pi \in\Pi_{\exp}$. The policy class $\Pi_{\exp}$ is an exploration policy class, described in more detail below. The learner does not incur any cost during the exploration episodes, and seeks only to gain information about the system. After the $N$ interaction episodes, it uses the collected data to propose a policy $\hat\pi \in \Pi^\star$. The learner is then evaluated on the expected cost of the proposed policy on a new evaluation episode. In particular, it incurs cost $\calJ(\hat \pi, \phi^\star)$. 

The policy classes $\Pi^\star$ and $\Pi_{\mathsf{exp}}$ are known; $\Pi^\star$ consists of deterministic policies, but $\Pi_{\mathsf{exp}}$ may be random. We do not assume $\Pi^\star = \Pi_{\mathsf{exp}}$.  We assume that the policy class $\Pi^\star$ has the parametric form:
\begin{align*}
    \Pi^\star = \curly{\pi^\theta \vert \theta \in \mathbb{R}^{d_{\theta}}}.
\end{align*}
No such parametric assumption is made on the exploration class $\Pi_{\exp}$. It instead  consists of whatever experimental procedures are available. For instance, it may be the class of policies with power or energy bounded inputs. Policies belonging to $\Pi_{\exp}$ must be history dependent (causal). We assume that the learner is allowed to randomly select choices of policies in $\Pi_{\exp}$.\footnote{i.e. for any $\pi^1, \pi^2\in\Pi_{\exp}$ and any $b \in [0,1]$, the policy $\pi_{\mix}$ which at the start of a new episode plays $\pi^1$ for the duration of the episode with probability $b$ and $\pi^2$ for the duration of the episode with probability $1-b$ also belongs to $\Pi_{\exp}$. }
Given these policy classes, the learning procedure should seek to identify the best exploitation policy belonging to $\Pi^\star$ by playing the most informative exploration policy in the class $\Pi_{\exp}$.

\subsection{Certainty Equivalent Control}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/Figures.pdf}
    \vspace{-18pt}
    \caption{Identfication to control pipeline. }
    \vspace{-18pt}
    \label{fig:CE pipeline}
\end{figure}

We focus on learners which follow a model-based approach to synthesize a control policy from interaction with the system, outlined in \Cref{fig:CE pipeline}. In this section, we discuss the learner's procedure for the last two steps: system identification and control synthesis.
In \Cref{s: main}, we return to the question of which experiments the learner should perform. 

Given the data collected during the experimentation phase, the learner finds an estimate for the dynamics by solving a nonlinear least squares problem. In particular, suppose that during the $N$ experimentation episodes of length $T$, the learner collects data $\curly{(U_t^n, X_t^n, X_{t+1}^n)}_{n,t=1}^{N, T+1}$. The subscript denotes the time index within each episode, while the superscript denotes the episode index. Using this dataset, the learner may identify the dynamics of the system by solving
\begin{align}
    \label{eq: least squares}
    \hat \phi \in \argmin_{\phi \in \R^{d_{\phi}}} \sum_{n=1}^N \sum_{t=1}^T \norm{X_{t+1}^n - f(X_t^n, U_t^n; \phi)}^2. 
\end{align}
Solving this problem provides a parameter estimate which is an effective predictor under the distribution of states and inputs seen during the experimentation. This notion can be captured via the prediction error. 

\begin{definition}
    We define $\ER_{\pi}^{\phi^\star}(\phi)$ as the prediction error for a parameter $ \phi$ under policy $\pi$: 
\begin{align*}
    \ER_{\pi}^{\phi^\star}( \phi) = \mathbb{E}_{\pi}^{\phi^\star} \left[ \frac{1}{T}\sum_{t=1}^T \norm{ f(X_t, U_t;  \phi) - f(X_t, U_t; \phi^\star) }^2 \right].
\end{align*}
\end{definition}

Once the learner estimates $\hat\phi$, the controller parameters are determined from the dynamics parameters by solving the policy optimization problem as
\begin{align}
    \theta^\star(\hat \phi) \in \argmin_{\theta \in \Re^{\dtheta}} J(\pi^\theta, \hat\phi). 
\end{align}
The certainty equivalent policy may then be expressed as a function of the estimated dynamics parameters $\hat\phi$ as
\begin{align}
    \label{eq: certainty equivalent policy}
    \pi^\star(\hat\phi) \triangleq\pi^{\theta^\star(\hat\phi)}.
\end{align}
We note that both the nonlinear least squares problem \eqref{eq: least squares} and the certainty equivalent control synthesis procedure of \eqref{eq: certainty equivalent policy} may be computationally challenging. The focus of this work is to understand the statistical complexity of the problem rather than the computational complexity. In the episodic setting we consider, both of these problems are solved offline. Therefore, given sufficient time and compute, it is often possible to determine good approximations to the optimal solutions using non-convex optimization solvers and approaches for policy optimization from the model-based reinforcement learning literature \citep{levine2020offline}.  



\subsection{Assumptions}

By \eqref{eq: certainty equivalent policy}, the optimal policy for the objective \eqref{eq: objective} under the true parameter $\phi^\star$ defining the dynamics \eqref{eq: dyn} is thus given by $\pi^\star(\phi^\star)$, and the corresponding objective value is $\calJ(\pi^\star(\phi^\star), \phi^\star)$. Meanwhile, the objective value attained under an estimate $\hat \phi$ is $\calJ(\pi^\star(\hat \phi), \phi^\star)$. We abuse notation and define the shorthand 
\begin{align}
    \label{eq: shorthand cost}
    \calJ_{\tilde\phi}(\phi) \triangleq \calJ(\pi^\star(\phi), \tilde\phi)
\end{align}
to describe the control cost of applying a certainty equivalence policy synthesized using  parameter $\phi$ on a system with dynamics described by $\tilde\phi$.  
It has been shown by \citet{wagenmaker2021task, wagenmaker2023optimal} that for models which are linear in the parameters, the gap $\calJ_{\phi^\star}(\phi) - \calJ_{\phi^\star}(\phi^\star)$ is characterized by the squared parameter error weighted by the \emph{model-task Hessian}, defined below.
\begin{definition}
    The \textit{model-task Hessian} for objective \eqref{eq: objective} and dynamics \eqref{eq: dyn} is given by 
    \begin{align*}
    \calH(\tilde \phi) = \nabla_{\phi}^2 \calJ_{\tilde\phi}(\phi)\vert_{\phi=\tilde\phi}, 
    \end{align*}
    where $\calJ_{\tilde\phi}$ is defined in \eqref{eq: shorthand cost}. 
\end{definition}
To express the excess cost achieved by a certainty equivalent controller synthesized using the estimated model parameters $\hat \phi$, we operate under the following smoothness assumption on the dynamics. 

\begin{assumption}(Smooth Dynamics)
    \label{asmp: smooth dynamics}
    The dynamics are four times differentiable with respect to $u$ and $\phi$. Furthermore, for all $(x,u) \in \R^{\dx} \times \R^{\du}$, all $\phi \in \R^{d_{\phi}}$, and $i, j \in \curly{0,1,2,3}$ such that $1\leq i+j \leq 4$, the derivatives of $f$ satisfy  
    \begin{align*}
        \norm{ D_{\phi}^{(i)} D_{u}^{(j)} f(x,u;\phi)}_\op \leq L_f.
    \end{align*}
\end{assumption}
The above assumption is satisfied for, e.g., control-affine dynamics which depend smoothly on $\phi$: $f(x_t, u_t; \phi) = g_1(x_t;\phi) + g_2(u_t; \phi) u$, with $g_1$ and $g_2$ each three time differentiable with respect to $\phi$. In this example, differentiability with respect to $u$ is immediate from the affine dependence. 

We also require that the policy class $\Pi^\star$ is smooth. 
\begin{assumption}(Smooth Policy Class)
    \label{asmp: smooth policy class}
    For $t=1,\dots, T$, $x \in \calX$, and any policy $\pi \in\Pi^\star$, the function $\pi_t^\theta(x)$ is four-times differentiable in $\theta$. Furthermore, $\norm{D_{\theta}^{(i)} \pi_t^\theta(x)}_{\op} \leq L_{\theta}$ for $i=1,\dots, 4$, $\theta \in \Re^{\dtheta}$, $x \in \calX$, and $t=1,\dots, T$. 
\end{assumption}
Note that such smoothness conditions are not imposed for the exploration policy class $\Pi_{\exp}$. The exploration policy class could, for instance, consist of model predictive controllers with constraints on the injected input energy, which do not satisfy such smoothness assumptions.

We additionally require that the costs are bounded for policies in the class $\Pi_{\star}$ and all dynamics parameters in a neighborhood of the true parameter. 
\begin{assumption}(Bounded Costs)
    \label{asmp: bounded costs}
    There exists some $r_{\cost}(\phi^\star) > 0$ such that for all $\phi \in \calB(\phi^\star, r_{\cost}(\phi^\star))$, and all $\pi \in \Pi^\star$, we have $\Ex_{\pi, \phi}\brac{\paren{\sum_{t=1}^T c_t(X_t, U_t) + C_{T+1}(X_T)}^2} \leq L_{\cost}$.
\end{assumption}
Due to the smoothness assumptions on the dynamics (Assumption~\ref{asmp: smooth dynamics}) and the policy class (Assumption~\ref{asmp: smooth policy class}),  the above assumption holds if the stage costs $c_t$ are smooth. 

We additionally suppose that  $\Pi^\star$ is not overparametrized. 
\begin{assumption}
    \label{asmp: unique optimal policy}
    The global minimum of $\calJ(\pi^\theta, \phi^\star)$, $\theta^\star(\phi^\star)$, is unique and satisfies $\nabla^2_\theta \calJ(\pi^\theta, \phi^\star)\vert_{\theta = \theta^\star(\phi^\star)} \succ 0$.
\end{assumption}
The above condition requires that there are a unique set of optimal control parameters for the true system.\footnote{To gain an intuition for this condition, observe that it holds for linear quadratic regulators as long as the input penalty matrix is positive definite.}


Under the above assumptions, we may show that the certainty equivalent policy is smooth near the optimal solution. 
\begin{lemma}[Proposition 6 of  \citet{wagenmaker2023optimal}]
    \label{lem: smooth policy}
    There exists some $r_{\theta}(\phi^\star) > 0$ such that for all $\phi \in \calB(\phi^\star, r_{\theta}(\phi^\star))$,
    \begin{itemize}[leftmargin=*]
        \item $\nabla_{\theta} \calJ(\pi^
        \theta, \phi)\vert_{\theta = \theta^\star(\phi)}=0$ 
        \item $\theta^\star(\phi)$ is three times differentiable in $\phi$ and  $\norm{D_{\phi}^i \theta^\star(\phi)}_{\op} \!\leq\! L_{\pi^\star}$ for some $L_{\pi^\star} > 0$ and $i \in \curly{1,2,3}$. 
    \end{itemize}
\end{lemma}

In order to bound the parameter recovery error in terms of the prediction error, additional identifiability conditions are needed. The following definition of a Lojasiewicz exploration policy is determined from a Lojasiewicz condition that arises in the optimization literature that measures the sharpness of an objective near its optimizer \citep{roulet2017sharpness}. In our setting, it quantifies the degree of identifiability from using a particular exploration policy. It does so by bounding the growth of identification error as a polynomial of prediction error. 
\begin{definition} [Lojasiewicz condition, \citet{roulet2017sharpness}]\label{def: loja}
For positive numbers $C_{\loja}$ and $\alpha$, we say that a policy $\pi\in\Pi_{\exp}$ is $(C_{\loja}, \alpha)$-Lojasiewicz if 
\begin{align*}
    \norm{\hat \phi - \phi^\star} \leq C_{\loja} \ER_{\pi}^{\phi^\star}(\hat \phi)^\alpha.
\end{align*}
\end{definition}

% \Bruce{include examples and figures of such a loss along with a Loja lower bound}

To ensure parameter recovery is possible for the learner, we make the following assumption regarding identifiability. 
\begin{assumption}
    \label{asmp: loja}
    Fix some positive constant $C_{\loja}$ and $\alpha \in (\frac{1}{4}, \frac{1}{2}]$. The learner has access to a policy $\pi^0 \in \Pi_{\exp}$ which is $(C_{\loja}, \alpha)$-Lojasiewicz.
\end{assumption}


While the Lojasiewicz assumption ensures that the data collected via the exploration policy $\pi^0$ is sufficient to identify the parameters, the rate of recovery may be slow. To bypass this limitation, we assume that some policy in the exploration class  satisfies a persistence of excitation condition. Persistence of excitation for a nonlinear dynamical system involves the positive definiteness of the following matrix:
\begin{align}
    \label{eq: covariance def}
    \Sigma^\pi \triangleq \E_{\pi}^{\phi^\star}\brac{\sum_{t=1}^T Df(X_t, U_t, \phi^\star)^\top D f(X_t, U_t, \phi^\star)},
\end{align}
 where $D f(X_t, U_t, \phi^\star)$ is the Jacobian of $f$ with respect to $\phi$ evaluated at $\phi^\star$. 
\begin{assumption}
    \label{asmp: good policy}
    There exists a policy $\pi \in \Pi_{\exp}$ for which
    \begin{align*}
        \E_{\pi}^{\phi^\star}\brac{\sum_{t=1}^T Df(X_t, U_t, \phi^\star)^\top D f(X_t, U_t, \phi^\star)} \geq \lambda_{\min}^\star > 0,
    \end{align*}
\end{assumption}

Finally, we make an assumption that all models parameters are relevant to perfect control.
\begin{assumption}
    \label{asmp: pd mt hessian}
    The model-task Hessian is positive definite:  $\calH(\phi^\star) \succ 0$.
\end{assumption}

The above assumption is quite strong, and does not hold for common baseline problems such as the linear-quadratic regulator with fully unknown dynamics matrices. However, this assumption is made primarily for ease of exposition. It can be removed in the linear setting at the expense of an algorithm which is more complicated to express concisely \citep{wagenmaker2023optimal}. The same approach used to bypass this condition in the linear setting can be easily extended to the nonlinear setting considered in this paper. We do not formalize this here, although we will in future work. 

\section{Proposed Algorithm and Main Result}
\label{s: main}

The above smoothness assumptions allow us to characterize the excess control cost of a policy synthesized via  certainty equivalence  applied to  a parameter estimate $\hat\phi$, \eqref{eq: certainty equivalent policy}. 
\begin{lemma}[Thm. 1 of  \citet{wagenmaker2023optimal}]\footnote{Thm. 1 of \citet{wagenmaker2023optimal} holds for systems with linear dependence on the unknown parameters; however it generalizes with minimal modification to the proof. See \Cref{s: smooth systems}.}
    \label{lem: cost decomposition}
    Suppose Assumptions~\ref{asmp: smooth dynamics}-\ref{asmp: unique optimal policy} hold. Let $r_{\theta}(\phi^\star)$ be as defined in \Cref{lem: smooth policy}.
    Then for $\hat\phi \in \calB(\phi^\star, \min\curly{r_{\cost}(\phi^\star), r_{\theta}(\phi^\star)})$, 
    \begin{align}
            \label{eq: excess cost as parameter error}
            \calJ_{\phi^\star}(\hat\phi)\! -\! \calJ_{\phi^\star}(\phi^\star)\! \leq \!\norm{\hat \phi \!-\! \phi^\star}^2_{\calH(\phi^\star)} +  C_{\cost} \norm{\hat \phi \!-\! \phi^\star}^3,
        \end{align}
        where $\calJ_{\phi^\star}(\phi)$ is as defined in \eqref{eq: shorthand cost} and
        \begin{align*}
            C_{\cost} = \mathsf{poly}(L_{\pi^\star},  L_f, L_{\theta}, L_{\cost}, \sigma_w^{-1}, T, \dx).
        \end{align*}
\end{lemma} 

\Cref{lem: cost decomposition} informs us that the leading term of the excess cost is given by the parameter estimation error weighted by the model-task Hessian, $\norm{\hat\phi-\phi^\star}_{\calH(\phi^\star)}^2$. 

Asymptotically, the distribution of the parameter estimation error is normally distributed with mean zero, and covariance given by the inverse Fisher Information matrix under the data collection policy $\pi$ evaluated at the true parameter value (cf. Theorem 1 of  \citet{lennart1980asymptotic}):
    \begin{align*}
        \lim_{N\to\infty} \sqrt{N} \FI^\pi(\phi^\star)^{1/2} (\hat \phi - \phi_\star) \sim \calN(0, I),
    \end{align*}
    where the Fisher information for the parameter $\phi$ under the policy $\pi$ for the model \eqref{eq: dyn} is given as
    \begin{align}
        \label{eq: fisher info}\FI^\pi(\phi)\!=\!\frac{\E_{\pi}^{\phi} \brac{\sum_{t=1}^T \!D f(X_t, U_t, \phi)^\top \!D f(X_t, U_t, \phi) }}{\sigma_w^2},
    \end{align} and measures the signal-to-noise ratio of the data collected from an episode of interaction with the system under the exploration policy $\pi$. 

We provide a novel non-asymptotic result which characterizes the $H$-norm of the parameter error for a positive definite matrix $H$ in terms of the Fisher Information matrix. 
\begin{theorem}
    \label{thm: identification error bound}
    Suppose Assumption~\ref{asmp: smooth dynamics} holds. Let $H$ be a positive definite matrix and let $\delta \in (0, \frac{1}{4}]$. Consider the least squares estimate $\hat\phi$ determined from \eqref{eq: least squares} using data collected from $N$ episodes via an exploration policy $\pi$ which is $(C_{\loja}, \alpha)$-Lojasiewicz for some $\alpha \in (\frac{1}{4}, \frac{1}{2}]$, and satisfies $\lambda_{\min}\paren{\Sigma^\pi} > 0$, with $\Sigma^\pi$ as defined in \eqref{eq: covariance def}. There exists a polynomial $\texttt{poly}_{\alpha}$ depending only on $\alpha$ such that the following condition holds. With probability at least $1-\delta$, 
    \begin{align}
        \label{eq: id error}
         \norm{\hat \phi - \phi^\star}_H^2 &\leq   40 \log \frac{24 d_{\phi}}{\delta} \frac{\trace(H \FI^\pi(\phi^\star)^{-1}) }{N} 
    \end{align}
    as long as
    \begin{align*}
        N &\geq \mathsf{poly}_\alpha\bigg(T,L_f,  d_{\phi}, \dx,  \sigma_w, \log N,  \log\frac{1}{\delta}, \log B_f, C_{\loja} \bigg).
    \end{align*}
\end{theorem}

By substituting the inequality \eqref{eq: id error} into the leading term of \eqref{eq: excess cost as parameter error}, one would expect that the the excess cost of deploying the certainty equivalent policy synthesized on a least squares estimate determined from data collected using policy $\pi$ is characterized by 
\begin{align}
    \label{eq: error charcterizing quantity}\trace(\calH(\phi^\star) \FI^\pi (\phi^\star)^{-1}).
\end{align}
In light of this, we would like to choose the exploration policy $\pi$ which minimizes this upper bound:
%the choice of exploration policy $\pi$ which minimizes this upper bound is 
\begin{align}
    \label{eq: ideal experiment design}
    \pi = \argmin_{\tilde \pi \in \Pi_{\exp}} \trace(\calH(\phi^\star) \FI^{\tilde \pi} (\phi^\star)^{-1}).
\end{align}
Our main result  shows that the above intuition can be made rigorous through careful analysis and design of the exploration policy. It then proceeds to show that we can find an exploration policy approximately solving \eqref{eq: ideal experiment design}, even though the parameter $\phi^\star$ defining the exploration objective is unknown prior to experimentation. 

To circumvent the issue of the unknown parameter $\phi^\star$, we consider a two step approach in which we first obtain a crude parameter estimate, and then refine it by playing a targeted exploration policy. Denote the crude estimate by $\hat\phi^-$.  This parameter can be used to search for a policy that approximately solves the optimization problem in \eqref{eq: ideal experiment design}. The straightforward approach to do so is to solve the problem under the estimated parameter: 
\begin{align}
    \label{eq: approximate exp design}
    \pi = \argmin_{\tilde \pi \in \Pi_{\exp}} \trace(H(\hat \phi^{-}) \FI^{\tilde \pi}(\hat \phi^-)^{-1}). 
\end{align}
While such a strategy may be effective if the coarse estimate is sufficiently close to the ground truth, it contends with the challenge that there is a distribution shift between the setting that the exploration policy is optimized for, and that which it is deployed in. In particular, $\FI^{\tilde \pi}(\hat \phi^{-1})$ pertains to the statistics from rolling out the dynamics under a parameter value different from the ground truth. We therefore instead consider the following problem: 
\begin{align}
    \label{eq: experiment design}
     &\pi = \argmin_{\tilde\pi \in \Pi_{\exp}} \trace\paren{H(\hat \phi^-) \Lambda_{\tilde\pi}^{-1}} \mbox{ where } \\
     \label{eq: Gram matrices}
     &\Lambda_{\tilde\pi} \!=\! \E_{\tilde \pi}^{ \phi^\star}\!\brac{\sum_{t=1}^TD f(X_t,U_t; \hat \phi^-)^\top D f(X_t,U_t; \hat \phi^-) }
\end{align}
Note the difference between \eqref{eq: approximate exp design} and \eqref{eq: experiment design}. In \eqref{eq: approximate exp design}, the Fisher information is determined using an expectation under the the dynamics parameter estimate $\hat\phi^-$ (see \eqref{eq: fisher info}). In contrast, the expectation in \eqref{eq: experiment design} is evaluated under the true parameter $\phi^\star$. If \eqref{eq: experiment design} can be optimized over the exploration policies, it alleviates the aforementioned  distribution shift issue. 

A minimizer for the above objective \eqref{eq: experiment design} may be approximated via an online learning procedure, as was recently proposed by \citet{wagenmaker2023optimal} for models that are linear in the parameter. In particular, we leverage the dynamic optimal experiment design ($\texttt{DOED}$) procedure proposed in the aforementioned work. For the reader's convenience, we state the algorithm and highlight several modifications in \Cref{s: doed}. We refer to our modified version of the algorithm as $\texttt{DOED}_+$. 

The above discussion motivates \Cref{alg: ALCOI}, named Active Learning for Control-Oriented Identification ($\texttt{ALCOI}$). The algorithm takes as input an initial policy satisfying the Lojasiewicz condition (Assumption~\ref{asmp: loja}), the exploration policy class, the target policy, the number of exploration rounds, and the desired confidence parameter $\delta$. Given these  components, the algorithm proceeds in three stages. The first stage begins in \Cref{line: intial policy} by playing the initial policy for one fourth of the exploration budget. In \Cref{line: coarse estimate}, it uses the collected data to derive a coarse estimate $\hat \phi^-$ for the unknown parameters by solving a least squares problem. Then, in \Cref{line: cnofidence ball} it constructs a confidence ball $\calB^-$ centered at $\hat \phi^-$:
\begin{equation}
\label{eq: confidence ball}
 \begin{aligned}
\calB^- &= \bigg\{\phi: \norm{\phi - \hat \phi^-} \leq \frac{R}{N^\alpha}\bigg\},
\end{aligned}   
\end{equation}
where
\begin{align}
    \label{eq: conf ball radius}
    R = \paren{\frac{2048 \sigma_w^2}{T } \paren{\dx +d_{\phi}\log\paren{L_f T N} + \log\frac{1}{\delta}}}^{\alpha}.
\end{align}
Next, the estimate $\hat \phi^-$ is used to construct the model-task Hessian at $\hat\phi^-$ as $\calH(\hat \phi^-)$. This is in turn used to define an exploration objective, $\Phi: \R^{d_{\phi} \times d_{\phi}} \to \R$ to be passed to the $\texttt{DOED}_+$ algorithm. This exploration objective  is a regularized version of that in \eqref{eq: experiment design} which takes as input a Gram matrix $\Lambda$, and outputs $\trace(\calH(\hat\phi^-) (\Lambda + \lambda I)^{-1})$. Here $\lambda > 0$ is a regularizer chosen from the estimate of the model-task Hessian in \Cref{line:regularizer}. 
The quantity $B_{\Phi}$ is then defined from the model-task Hessian and the regularizer to characterize the smoothness of the objective $\Phi$. The exploration objective is passed to $\texttt{DOED}_+$ along with the coarse estimate $\hat \phi^-$, the ball $\calB^-$ and the smoothness bound $B_{\Phi}$ in \Cref{line: doed call}. This call to $\texttt{DOED}_+$ returns a collection of $\tilde K$ policies, where $\tilde K$ is a polynomial function of the supplied budget; see \Cref{s: doed} for further details. The mixture of the returned policies approximately minimizes the exploration objective $\Phi$ over Gram matrices of the form \eqref{eq: Gram matrices}, thereby approximating a solution to \eqref{eq: experiment design}.  We therefore use them to design a mixture policy which plays any of the returned policies with equal probability, and plays the initial exploration policy $\pi^0$ with probability $\frac{1}{2}$.\footnote{The initial policy $\pi^0$ included in $\pi_\mix$ to ensure that $\pi_{\mix}$ is a $(2C_{\loja}, \alpha)$-Lojasiewicz policy. } This policy is run to collect data from the system, and obtain a fresh estimate $\hat\phi^+$ for $\phi^\star$.\footnote{In practice, one  would use all of the the data to estimate $\hat\phi^+$. However, using only the data from an independent rollout contributes only a constant factor to the rate, and simplifies the analysis.} Finally, the estimate is used to synthesize the certainty equivalent policy as in \eqref{eq: certainty equivalent policy}.

\begin{algorithm}
\caption{$\texttt{ALCOI}(\pi^0, \Pi_{\exp}, \Pi^\star, N, \delta)$} 
\label{alg: ALCOI}
\begin{algorithmic}[1]
\State \textbf{Input:} Initial policy $\pi^0$, exploration policy class $\Pi_{\exp}$, target policy class $\Pi^\star$, episodes $N$, confidence $\delta$. 
\State \label{line: intial policy} Play $\pi^0$ for $\lfloor \frac{N}{4} \rfloor$ episodes to collect $\curly{X_t^n, U_t^n, x_{t+1}^n}_{t, k=1}^{T, \lfloor \frac{N}{4} \rfloor}$.
\State \label{line: coarse estimate} Fit $\hat \phi^-$ from the collected data by solving \eqref{eq: least squares}.
\State \label{line: cnofidence ball} Set $\calB^-$ according to \eqref{eq: confidence ball}.
\State \label{line:regularizer} Set $\lambda \gets \frac{\lambda_{\min}(\calH(\hat\phi^-)) \lambda_{\min}^\star}{16 \norm{\calH(\hat\phi^-)}_{\op} d_{\phi}}$.
\State \label{line: exp design obj} Define objective 
$\Phi(\Lambda) \gets \trace(\calH(\hat\phi^-) (\Lambda+\lambda I)^{-1})$. 
\State \label{line: smoothness bound} Set objective smoothness bound $B_{\Phi} \gets \frac{T L_f^2 \norm{\calH(\hat\phi^-)}}{\lambda^2}$.
\State \label{line: doed call} Determine exploration policies as $\curly{\pi^k}_{k=1}^{\tilde K} \gets \texttt{DOED}_+(\Phi, \lfloor\frac{N}{4}\rfloor, \pi^0, \hat \phi^-,\calB^-, B_{\Phi})$.
\State \label{line: mix} Define $\pi_{\mix}$ which at the start of each episode plays $\pi^0$ with probability $\frac{1}{2}$, and for $i=1,\dots, \tilde K$ plays $\pi^i$ with probability $\frac{1}{2 \tilde K}$.
\State Play $\pi_{\mix}$ for $\lfloor N/2 \rfloor$ episodes, collecting data $\curly{X_t^n, U_t^n, X_{t+1}^n}_{t, k=1}^{T, \lfloor \frac{N}{2} \rfloor}$.
\State \label{line: fine model} Fit $\hat \phi^+$ by solving \eqref{eq: least squares} with the data $\curly{X_t^n, U_t^n, X_{t+1}^n}_{t, k=1}^{T, \lfloor \frac{N}{2} \rfloor}$.
\State \textbf{Return: } certainty equivalent policy $\hat \pi = \pi^\star(\hat \phi^+)$
\end{algorithmic}
\end{algorithm}
\setcounter{algorithm}{0}
\begin{algorithm}
\
\caption{$\texttt{ALCOI}(\pi^0, \Pi_{\exp}, \Pi^\star, N, T)$}
\begin{algorithmic}[1]
\State \textbf{Input:} Initial policy $\pi^0$, exploration policy class $\Pi_{\exp}$, target policy class $\Pi^\star$, episodes $N$, time horizon $T$
\State Play $\pi^0$ for $\lfloor \frac{N}{2} \rfloor$ episodes, and fit LS estimate $\hat \phi^-$
\State Let $\pi_{\mathsf{exp}}$ be  a $\varepsilon$-optimal solution for $\inf_{\pi \in \Pi_{\mathsf{exp}}} \trace(H(\hat \phi^-) \mathsf{FI}^{\pi_{\mathsf{exp}}}(\hat \phi^-)^{-1}) $ \\
// Analysis uses a slightly different objective - see paper
\State Play $\pi_{\exp}$ for $\lfloor \frac{N}{2} \rfloor$ episodes and fit LS estimate $\hat \phi^+$
\State \textbf{Return: } CE policy $\hat \pi = \hat \pi(\hat \phi^+)$
\end{algorithmic}
\end{algorithm}

Our main result is a finite sample bound characterizing the excess cost of the policy return by \Cref{alg: ALCOI}. 
\begin{restatable}[Main Result]{theorem}{mainresult}\label{thm: main}
Suppose $f$, $\pi^0$, $\Pi_{\exp}$, $\Pi^\star$ satisfy Assumptions~\ref{asmp: smooth dynamics}-\ref{asmp: pd mt hessian}. Let $\delta \in (0,\frac{1}{4}]$.
Consider running \Cref{alg: ALCOI} to generate a control policy $\hat\pi$ as $\hat \pi = \texttt{ALCOI}(\pi^0, \Pi_{\exp}, \Pi^\star, N, \delta)$. 
There exists a universal positive constant $c$ and polynomial function $\texttt{poly}_\alpha$ depending only on the Lojasiewicz parameter $\alpha$ such that the following holds true. 
With probability at least $1-\delta$ we have that
\begin{align*}
    &\calJ(\hat \pi, \phi^\star) \!-\!  \calJ_{\phi^\star}(
\phi^\star) \leq c \frac{\log\frac{d_{\phi}}{\delta}}{N} \!\min_{\tilde \pi \in \Pi_{\exp}}\! \trace\paren{\calH(\phi^\star) \FI^{\tilde \pi}(\phi^\star)^{-1} },
\end{align*}
as long as 
\begin{align*}
    N \!&\geq \!\mathsf{poly}_\alpha\bigg(\!T,L_f, L_{\cost},  L_{\pi^\star}, d_{\phi}, \dx, \frac{1}{\lambda_{\min}^\star}, r_{\cost}(\phi^\star), r_{\theta}(\phi^\star)\\&\frac{1}{\lambda_{\min}(\calH(\phi^\star))}, \norm{\calH(\phi^\star)}, \sigma_w, \log N,  \log\frac{1}{\delta}, \log B_f, C_{\loja} \bigg).
\end{align*}
\end{restatable}

The above result characterizes the excess control cost in terms of three key quantities. First, the term $\calH(\phi^\star)$ is the model-task Hessian, which describes how error in identification of the dynamics model parameters translates to the control cost. Second, is the inverse Fisher Information of the optimal exploration policy term, which measures a signal-to-noise ratio quantifying the hardness of parameter identification. Finally, the number of exploration episodes $N$ on the denominator captures the rate of decay from increasing the experimental budget. 

We note that in the setting where the dynamics model has linear dependence on the parameters, \citet{wagenmaker2023optimal} present a lower bound on the excess control cost achieved by any learner following the model based interaction protocol described in \Cref{s: problem formulation}. The upper bound of \Cref{thm: main} matches this lower bound up to universal constants, and the log term $\log\paren{d_{\phi}/\delta}$. Future work will pursue general lower bounds that hold for dynamics models with a nonlinear dependence on the unknown parameter. We conjecture that in general, the upper bounds of \Cref{thm: main} are tight up to universal constants and the term $\log\paren{d_{\phi}/\delta}$. 

We note that the burn-in time is currently polynomial in the relevant system parameters; however, we do not pursue tight burn-in times in this work. It may be possible to improve the dependence of the burn-in on various system quantities, e.g. by leveraging stability or reachability to obtain optimal dependence of the burn-in on $T$. 

\section{Proof Sketch}
\label{s: pf sketch}

Full proof details may be found in the appendix. Here, we present a sketch. Our main result proceeds by demonstrating the following sub-steps. In these sub-steps, let $C$ be a polynomial of the problem parameters, as in the burn-in requirement of \Cref{thm: main}. 
\begin{enumerate}[noitemsep,nolistsep,leftmargin=*]
    \item \label{item: coarse id bound} The coarse parameter estimation error decays gracefully with the total amount of data:
    \begin{align}
        \label{eq: coarse estimation error}
        \norm{\hat\phi^--\phi^\star} \leq \frac{C}{(TN)^{\alpha}},
    \end{align}
   as long as $N$ exceeds some polynomial burn-in time.  This result is derived from recent results characterizing non-asymptotic bounds for identification \citep{ziemann2022learning}, and takes the place of the estimator consistency requirements in classical asymptotic identification literature \citep{lennart1980asymptotic}. By making the number of episodes $N$ sufficiently large, we can make this error arbitrarily small. It thus characterizes a type of ``consistency burn-in''. 
   \item \label{item: coarse approx of exp design} As long as the coarse estimation error of \eqref{eq: coarse estimation error} is sufficiently small, the ideal optimal exploration objective of \eqref{eq: ideal experiment design} is well-approximated by the objective \eqref{eq: experiment design}. In particular, for any exploration policy $\pi\in\Pi_{\exp}$,
   \begin{equation}
   \label{eq: ideal to approx exploration}
   \begin{aligned}
       \!&\bigg|\!\trace\paren{\!\calH(\hat \phi^-) \Lambda_\pi^{-1}\!}\! -\!\trace(\calH(\phi^\star) \FI^{\pi} (\phi^\star)^{-1}) \bigg|\! \leq \!C\! \norm{\hat\phi^- \!\!- \!\phi^\star}, 
   \end{aligned}
   \end{equation}
   with $\Lambda_\pi$ as in \eqref{eq: Gram matrices}.
   \item \label{item: doed call} The call to the $\texttt{DOED}_+$ algorithm in \Cref{line: doed call} of \Cref{alg: ALCOI} returns a collection of policies whose mixture approximately minimizes the exploration objective \eqref{eq: experiment design}:
   \begin{equation}
       \label{eq: doed success}
   \begin{aligned}
       &\trace\paren{\calH(\hat \phi^-)\Lambda_{\pi_{\mix}}^{-1}} \leq \frac{C}{N^\alpha} \!+\!  \min_{\tilde\pi\in\Pi_{\exp}}\trace\Bigg(\calH(\hat \phi^-) \Lambda_{\tilde\pi}^{-1}\Bigg),
   \end{aligned}
   \end{equation}
   for $\Lambda_{\pi}$ as in \eqref{eq: Gram matrices}. Demonstrating this result involves specializing the dynamic optimal exploration algorithm and its proof of correctness to our setting from \citet{wagenmaker2023optimal}. %The modifications to the algorithm are shown in \Cref{s: doed}.
   \item \label{item: sysid bnd} For $N$ sufficiently large, we may use the consistency guarantee  \eqref{eq: coarse estimation error} to prove \Cref{thm: identification error bound}. % for any policy $\pi$ that is persistently exciting (i.e. any policy such that $\Sigma^\pi$, defined in \eqref{eq: covariance def}, is positive definite). 
   The proof of this fact follows by revisiting the delta method \citep{van2000asymptotic} through the lens of concentration inequalities. Doing so results in the near sharp\footnote{Rates matching the  asymptotic limit up to logarithmic factors.} rates we obtain. 
\end{enumerate}
Using the above results, our argument proceeds according to the following series of inequalities applied to the excess cost:
\begin{equation}
\label{eq: excess cost pf}
\begin{aligned}
    &\calJ_{\phi^\star}(\hat\phi^+)  \!-\! \calJ_{\phi^\star}(\phi^\star) \leq \norm{\hat\phi^+ - \phi^\star}_{\calH(\phi^\star)}^2 \!+\! C_{\cost} \norm{\hat\phi^+ - \phi^\star}^3 \\
    &\leq 40\log\paren{ \frac{ 24 d_{\phi}}{\delta}} \frac{\trace(\calH(\phi^\star) \FI^{\pi_{\mix}}(\phi^\star)^{-1}) }{N} + \frac{C}{N^{3/2}},
\end{aligned}
\end{equation}
where the first inequality follows by \Cref{lem: cost decomposition}, and the second inequality follows by applying \Cref{thm: identification error bound} with $H=\calH(\phi^\star)$ for the first term, and $H=I$ for the second term\footnote{The condition that $\Sigma^{\pi_\mix} \succ 0$ in \Cref{thm: identification error bound} can be shown from the success of $\texttt{DOED}$ in \eqref{eq: doed success}). }. Next, it follows that
\begin{align*}
    \trace(\calH(\phi^\star) \FI^{\pi_{\mix}}(\phi^\star)^{-1}) &\overset{(i)}{\leq}  \frac{C}{N^\alpha}  +  \trace\paren{H(\hat \phi^-) \E_{ \pi_{\mix}}^{ \phi^\star}\brac{(D f(x_t,u_t; \hat \phi^-))^\top D f(x_t,u_t; \hat \phi^-) }^{-1}}  \\
    &\overset{(ii)}{\leq}  2\frac{C}{N^\alpha} +  \min_{\tilde\pi\in\Pi_{\exp}}\trace\Bigg(H(\hat \phi^-) \E_{\tilde\pi}^{ \phi^\star}\brac{(D f(x_t,u_t; \hat \phi^-))^\top D f(x_t,u_t; \hat \phi^-) }^{-1}\Bigg) \\
       &\overset{(iii)}{\leq} 3\frac{C}{N^\alpha} +  \min_{\tilde\pi\in\Pi_{\exp}}\trace\Bigg(H(\phi^\star) \FI^{\tilde\pi}(\phi^\star)^{-1}\Bigg),
\end{align*}
where inequality $(i)$ follows from \eqref{eq: ideal to approx exploration} and \eqref{eq: coarse estimation error}, inequality $(ii)$ follows from \eqref{eq: doed success}, and inequality $(iii)$ follows from \eqref{eq: ideal to approx exploration} and \eqref{eq: coarse estimation error}. The main result then follows by substituting the above bound into \eqref{eq: excess cost pf}, and taking $N$ to exceed a polynomial burn-in time so the higher order terms become negligible. 


